Model-diff: A Tool for Comparative Study of Language Models in the Input Space

Comparing two (large) language models (LMs) side-by-side and pinpointing their prediction similarities and differences on the same set of inputs are crucial in many real-world scenarios, e.g., one can test if a licensed model was potentially plagiarized by another. Traditional analysis compares the LMs' outputs on some benchmark datasets, which only cover a limited number of inputs of designed perspectives for the intended applications. The benchmark datasets cannot prepare data to cover the test cases from unforeseen perspectives which can help us understand differences between models unbiasedly. In this paper, we propose a new model comparative analysis setting that considers a large input space where brute-force enumeration would be infeasible. The input space can be simply defined as all token sequences that a LM would produce low perplexity on -- we follow this definition in the paper as it would produce the most human-understandable inputs. We propose a novel framework \our that uses text generation by sampling and deweights the histogram of sampling statistics to estimate prediction differences between two LMs in this input space efficiently and unbiasedly. Our method achieves this by drawing and counting the inputs at each prediction difference value in negative log-likelihood. Experiments reveal for the first time the quantitative prediction differences between LMs in a large input space, potentially facilitating the model analysis for applications such as model plagiarism.

==> 2methodnew.tex <==
\section{Preliminaries}

\subsection{Output Distribution of Models}
% introduce basics, using CV/ML terminologies is fine

\subsection{Parallel Tempering and Histogram Reweighing}
% introduce the prior work, based on the terms in the previous section

\subsection{Language Models}
% introduce language models, next token prediction, input, output vocabulary/tokenizer.


\section{Method}
% first talk about the problem, the difference of language models to traditional models, and the necessity of auto-eval and model-diff. Highlight the contributions: (1) model eval of LMs, (2) auto-eval, (3) model-diff.

==> intro_back.tex <==

\section{Introduction}
%\zihan{Overall, I think we need a figure or something to illustrate what predictive difference looks like. Imagine someone is using this tool to compare, what would the user interface look like?}

It is crucial in many real-world scenarios to compare two (large) language models (LMs) side-by-side and pinpoint their prediction differences. For example, the prediction differences may help identify which model agrees more with human annotations; it can also identify model plagiarism between a licensed open-sourced model and its small variate version whose weights are added small noise. 
% Traditional analysis is dataset-driven, where a dataset is first crafted and then used to compare the two LMs. 
% However, the dataset is usually built for some designed perspectives (e.g., math), and would not be generic enough to cover the unforeseen ones (e.g., whether the model is good at making poems). 
% While a current trend is to construct datasets from different perspectives brainstormed by researchers and engineers or proposed by customers, an underlying dilemma pertains --- to faithfully compare models, wei{the model should not be exposed to the underlying dataset which contains high quality data that would otherwise be beneficial for model training}.
% % We argue that this is unavoidable if the comparison is dataset-driven.
% Retrospectively, model comparison is essentially about understanding how models differ in handling inputs.
% If computation were not a problem, we would enumerate all the inputs, subsample the ones we care about (e.g., human-readable ones) and observe the ones where the models behave differently.
% In turn, if we broadly define the behavior as the LM's negative log likelihood of its next token prediction task on the input, we could also apply sampling-based methods to obtain samples of different behaviors (different NLL). 
% \wei{Sampling is efficient, however, the underlying distribution that is (usually exponentially) biased to low NLL, compared to the uniform enumeration.
% Therefore, the result based on sampling would be hard to interpret.
% In this work, we pioneer an efficient and unbiased (to the uniform enumeration) comparison framework for models. }
% We achieve this by integrating a correction mechanism during sampling (\zihan{can help me explain PTHR better}), and normalization post-sampling.
% We are able to obtain both unbiased samples on different (NLL) prediction differences, and statistics that would aid the comparison. 
% \zihan{After this, we dive in and explain our method in detail}
Traditional analysis compares the LMs' outputs on the same benchmark dataset which only covers a limited number of inputs from their designed perspectives.
However, (large) LMs
%\jingbo{I don't think we want to mention agent here. This work is not specific to agent. As a motivation, we only need to claim that there are many LMs are deployed. Since we are focused on LMs, we should keep the scope as LM. } 
have recently been deployed online and widely accessible to the public. %, where the unanticipated and untested perspectives may present a challenge.
As users in principle can input %\jingbo{what does it mean ``virtually''? like ``users are supposed to''?} 
any types of data that could potentially cause the models to behave unexpectedly, it could be beneficial if we can assess models on this large amount of data with unforeseen perspectives to analyze the models.
%\jingbo{Do we have to emphasize ``equal importance'' here? I would hide it a bit here.}\wei{Do you mean to complete remove it or just don't use emph?}
%Traditional approaches that only cover the anticipated perspectives by datasets for prediction difference raise concern as they are not able to represent the use cases when the users can virtually input anything.
% \jingbo{The challenge/drawback of using benchmark datasets should be two folds: (1) the perspectives are limited by the number of datasets and (2) the number of inputs from the same perspective is limited by the dataset size. Shout these two out directly. And then talk about an input space --- like all token sequences that human would feel reasonable as an input.}
The challenge of using benchmark datasets in this case is twofold: (1) the tested perspectives are limited by the types of test sets, and (2) the variety of inputs from the same perspective is limited by the dataset size.

\begin{figure*}[ht]
  \centering
\includegraphics[width=0.85\linewidth]{figs/model-diff.png}
  %\vspace{-6mm}
  \caption{Overview of Model-diff with hypothetical models, code-LM (model $A$) and math-LM (model $B$).
  %\jingbo{this caption is too long. Is there any way to move some of the content to the pictures themselves? }
  (a) code-LM assigns ``i=i+1'' (circled in orange \mycircle) a small output value (z=NLL) but math-LM assigns a large NLL.
  (b) The set of inputs $\mathbb X_A$ ($\mathbb X_B$) that model $A$ ($B$) maps to a predefined output range $\mathbb Z=[z_-,z_+]$.
  The Output distributions $\rho_A(z)$ and $\rho_B(z)$ are the count of inputs at each $z$.
  (c) Using each model's prediction $z_{A,\mathbf{x}}$ and $z_{B,\mathbf{x}}$ as two coordinate axes indicates the relation of models' predictions of the same input (e.g. $z_{A,\mathbf{x}} < z_{B,\mathbf{x}}$ for ``i=i+1''). The number of inputs in R3 is used to normalize statistics for sampling (Sec.~\ref{sec:normalization}).  
  (d) Feeding the inputs in $\mathbb X_A$ to both models, compute each $\diff=z_{A,\mathbf{x}}-z_{B,\mathbf{x}}$, and count the number of inputs to get $\rho_{A\rightarrow B}(\diff)$ (red histogram). Repeat for model $B$ to get $\rho_{B \rightarrow A}(\diff)$ (light blue histogram). The ``i=i+1'' is mapped to a very negative $\diff$ value.
%\jingbo{what is R1, R2, and R3 in (b)? Shall we describe them using PA and PD terms? Shall we color R1, R2, R3 and the background areas following some pattern?}
}
  \label{fig:diff}
  \vspace{-3mm}
\end{figure*}

%\zihan{The traditional way to obtain xxx (we can use prediction difference for now, maybe we will come up of a better phrase later) is xxx. However, some difficulty...} 

%Shout these two out directly. And then talk about an input space --- like all token sequences that human would feel reasonable as an input.
In this paper, we propose to compare models with a large number of data, or more generally, in a (discrete) input space that is finite but computationally impossible to enumerate all inputs.
% , or more generally, on a (discrete) input space which is finite but computationally impossible to enumerate all the data points. 
% The input space is so large that it does not need to specify the perspectives to test.
% \wei{I use the word "One" as an example?} 
While the combination of all token sequences is a straightforward space, it is not ideal as most of them are sequences with random tokens, hence not beneficial for analysis. 
One reasonable input space is the collection of human-understandable inputs. 
It can be defined as all token sequences that an LM produces negative log-likelihood (NLL)\footnote{NLL is log-probability or log-perplexity which is the loss to train next token prediction for LMs.} within a range of small values.
Here we do not treat models as language generators but as language modeler, where a (good) language model is expected to output low NLL (low perplexity) to inputs of text sequences that humans see as reasonable and fluent, and high NLL (high perplexity) to inputs that are nonsensical or unreasonable.
We focus on this input space because the number of human-understandable sequences is large enough to cover the unforeseen perspectives and data to analyze the models.
%\wei{"We randomly sample from the comparisons to explicitly understand the differences. 
%Such process is automatic and can cover more unforeseen perspectives as we draw more random samples." These two sentences are great, but I feel like it might be too much to talk about sampling in this paragraph? Maybe we can better use them to this paragraph (as I did for the last sentence), and mention the other sentence in the next paragraph?} 
%\jingbo{sure, I like this idea.}
%\zihan{mention fixed length later in experiments, I don't think it is a fundamental drawback} 
%\zihan{probably don't need to exaplin log likelihood too much} 
% One reasonable input space to consider is the input space of any token sequences that human may feel as possible inputs, e.g., human readable.
% In this paper, we define this reasonable input space as all the token sequences of a fixed length that a LM believes to be reasonable human sequences reflected by a range of low negative log-likelihood .

% \wei{Alternative of this sentence: This reasonable input space is generally achieved as all the token sequences of a fixed length that a LM believes to be reasonable human sequences reflected by a range of low negative log-likelihood (NLL\footnote{NLL is log-probability or log-perplexity, which is the loss to train next token prediction for language models.}).}

% which achieve a perplexity within a certain range judged by a LM (e.g., GPT-2).
% For example, the input space could contain all the inputs 
 

%\zihan{We are putting too much in this sentence, can we split it into two parts, or even leave a less important part of it in a later paragraph?}

To tackle this new evaluation of a large input space, we propose a sampling-based comparative analysis framework, Model-diff, that can efficiently estimate the prediction difference for the \emph{types} and \emph{count} of the inputs at each level of the prediction difference value. 
%Sampling can cover more unforeseen perspectives as we draw more random inputs. 
Consider two hypothetical models %\jingbo{we can say they are LMs? Like LMs model the NLL of a sequence ... } 
that optimize the NLL loss. They are fine-tuned to domain tasks as code-LM %\jingbo{shall we call them code-LM? I don't know why it's called GPT?} 
(model $M_A$) and math-LM (model $M_B$). 
In Fig~\ref{fig:diff}(a), the types of inputs that code-LM predicts with a low NLL could be the variable assignment code such as ``i=i+1'', whereas math-LM thinks this text is a wrong math equation and thus assigns a high NLL (Fig~\ref{fig:diff}(b)).
If two models predict similar NLLs for each input in an input space, the count of prediction difference (e.g. $\diff=\text{NLL}_A-\text{NLL}_B$) concentrates around 0, indicating the models are similar.
Because the input space is not enumerable, we uniformly sample the input space to assess the prediction differences between the two models by scrutinizing the inputs and counting the number of inputs given different output values (e.g., there are 10 math equations when $\diff=-5$ and 23 code inputs when output is $\diff=10$ etc), similar to Fig~\ref{fig:diff}(d).
% \wei{I think here we need to clarify a little bit on the largest input space and the input space that model believes to be reasonable human inputs.} 
% \jingbo{Yes, we can start with the ``valid'' input space which includes all the token sequences based on the vocabulary, and then talk about the input space that a model believes to be reasonable human inputs. We can claim that the second input space is more intuitive and useful, giving the reviewers some feelings of our thinking process and hope they will appreciate this consideration.}
% \jingbo{Let's give it a notation or a name for ``the input space that a model believes to be reasonable human inputs'' so we can refer to it easily in the rest of the paper.}
% As the number of C++ commands or math equations is small in the input space that a model believes to be reasonable human inputs,
% it is rare and inefficient for uniform sampling to sample math equations or code commands as inputs. \wei{Or "But it is difficult to find an input space that the model believes to be reasonable human inputs."}

% recent works~\citep{booth2021bayes,liu2023omniinput} have shown that the choice of datasets affects the understanding and conclusions of models' prediction difference. They found sampling methods -- finding the inputs that are mapped to certain output values (e.g. low perplexities for language models) -- are preferable to prevent the biases from selecting and testing certain datasets~\cite{zeiler2014visualizing,
% ribeiro2016should,
% lundberg2017unified, ghorbani2019automating}. 

Model-diff samples the models whose predictions are within a range of low NLL. The outputs of sampling, including the sampled inputs and the count histogram that is processed to get the \emph{output distribution}, can be used to compare the types and counts of the inputs.
%\wei{sampling output distribution overcomes the efficiency. It gets the count and types of the inputs. }
%It leverages the output distribution of $\diff$ to compare the types and count of sampled inputs.
Output distribution~\citep{pmlr-v202-liu23aw}
%\jingbo{give a citation to our previous work}
is a distribution of the count of the inputs given each output value, the exact quantity for count comparison.  Comparing the summations of two models over this quantity for different output values can help compare the total \emph{count} of inputs in an input space even though the input space is usually too large to be enumerated.
Scrutinizing the sampled inputs for different outputs can help understand the \emph{types} of the inputs.  
Model-diff leverages them to quantify the agreed/disagreed predictions between the two models.
Moreover, to ensure a fair comparison, each model will propose its own input space with inputs of low NLLs and compare predictions by the other model. 
Model-diff involves a novel normalization strategy for the two output distributions 
%to fairly compare the prediction difference between the two different \tina{shouldn't be the prediction difference between the two difference input spaces? because even on the same input space you check how the two models evaluate them} 
in the input spaces proposed by each model.

%With this information, some applications of Model-diff could be to tell which model is better in terms of agreement to human predictions, or provides potential indication of model plagiarism.
% In practice, Model-diff consists of four steps:\wei{add section numbers.}
% \begin{enumerate}[nosep,leftmargin=*]
%     \item[(a)] We generate inputs of text by sampling model $A$'s meaningful output values $\mathbb Z$. This data generation process also collects the statistics (frequency histogram) that can compute output distribution $\rho_A(z)$ for $A$'s meaningful output value $z \in \mathbb Z$.    
%     \item[(b)] We feed each sampled input from $A$ to model $B$ to compute prediction (output) difference $\diff$. The $\diff$ of the sampled inputs from $A$ form a distribution $\rho_A(\diff)$~\footnote{This distribution is adjusted by the output distribution of the meaningful output values.} of prediction difference. $\rho_A(\diff)$ describes the count for each level of prediction difference $\diff$. 
%     \item[(c)] We repeat the same process to get $\rho_B(\diff)$ for model $B$.
%     \item[(d)] $\rho_A(\diff)$, $\rho_B(\diff)$, and the correspondent sampled inputs are compared and analyzed to quantify prediction difference.
% \end{enumerate}

% Compared to previous sampling-based model understanding and evaluation method equipped with output distribution~\cite{liu2023omniinput}, Model-diff proposes a new normalization method of output distributions without having to sample all the output values. 
% Compared to other model evaluation (comparison) methods that use generative models to generate data without using datasets~\cite{luo2023zeroshot,prabhu2023lance,shu2020identifying,leclerc20223db}, Model-diff compares the models only by sampling the models themselves for the output distributions and the correspondent representative inputs without using external (generative) models for data generation which could introduce biases. 

%\zihan{we probably can directly start with contributions, and detail each bullet point}
\paragraph{Contributions}
\begin{itemize}[nosep,leftmargin=*]
    \item We propose a new comparative analysis setting between two models by examining their prediction differences on the full input space, in contrary to leveraging crafted datasets of testing foreseen perspectives. %This setting benefits to detect model-plagiarism and determine better model in terms of agreement human annotation and model prediction in a much larger input space beyond datasets.  
    %\zihan{Better if we have serveral use cases in hand, so we can say the previous approach is unable to identify xxx}. 
    \item To address the infeasible compute time of enumeration, we propose Model-diff. It can help understand the \emph{type(s)} and the (relative) \emph{count} of the agreed/disagreed predictions between two models in the input space corresponding to meaningful output values.
    \item We confirmed the correctness of Model-diff through a Toy example. Further experiments show Model-diff can find prediction differences for GPT2 with various sequence lengths and Llama. Moreover, application to model plagiarism with Model-diff discovers distinctive patterns  for a model whose weights are added noise. This could be a useful signal for further investigation.
\end{itemize}
% As far as we know, Model-diff is the first that evaluates the prediction differences between two models in an input space that is too large to be enumerated.
% It reveals the first time the (relative) total count that the two models disagree/agree on each other's predicted NLL in an input space \wei{and shows several interesting findings: ``interesting'' triggers questions.}. 
% Our paper is a demonstration of how to use output distribution for comparative analysis
% that could be scaled when more advanced samplers and more computation (and human annotations) resources are available, instead of a conclusive study for different models. Our contributions are
% \begin{itemize}[nosep,leftmargin=*]
%     \item We propose that a model comparative setting between two models' in an input space which is too large to enumerate.
%     \item We develop a novel model comparative analysis framework, Model-diff. It can help understand the \emph{type(s)} and the (relative) \emph{count} of the agreed/disagreed predictions between two models in the input space corresponding to meaningful output values.
%     \item We apply Model-diff to evaluate popular pre-trained (large) language models. The results reveal new findings and insights of models' prediction difference.
% \end{itemize}



% all their inputs shall be considered as equally important, but it is generally too many inputs to enumerate in the space but some output values may have more inputs than the others, thereby making it hard to use the sampled inputs for prediction difference.  

% To study the prediction difference between two models using sampling instead of datasets, we propose Model-diff that can address the issue of relative total count for different output values during sampling. Model-diff first acquire (1) the (representative) inputs for different output values and (2) the output distribution -- how many inputs are mapped to certain output values -- for the two models to be compared with. It then samples each model's representative inputs by , we measure the difference in prediction between two models on each input within the , such as the $\text{NLL}-\text{NLL}$ for language models, and   

% Based on Once we get the two  

%\wei{OmniInput} \wei{cite} \wei{leverages the recently introduced output distribution for model understanding and comparison. However, many previous works including OmniInput constrain the input space by introducing another model thereby its biases. On the other hand, we believe that all the inputs correspond to meaningful output values are valid for model comparison, because the mapping inputs to those meaningful output values reflect model's biases which we are interested in analyzing.}  



% (a) code-LM assigns ``x=x+1'' a small output value (z=NLL) but math-LM assigns large output value because this is not a normal math equation.
%   (b) With many sampled inputs, we can acquire output distributions $\rho_A(z)$ and $\rho_B(z)$ for the two models within predefined output range $ \mathbb Z=[z_-,z_+]$ and the sampled inputs $\mathbf{x}_A$ (\mytri) from $A$ and $\mathbf{x}_B$ (\mysqua) from $B$. ``x=x+1'' (circled in orange \mycircle) is mapped within $\mathbb Z$ by $A$ but outside $\mathbb Z$ by $B$. 
% (c) Using each model's prediction $z_{A,\mathbf{x}}$ and $z_{B,\mathbf{x}}$ as two coordinate axes, we can identify the relation of models' predictions of the same input. For example, the circled input has a small $z_{A,\mathbf{x}}$ but a large $z_{B,\mathbf{x}}$. Regions $\text{R}_1+\text{R}_3$ indicates model $A$'s output is within $\mathbb Z$. Regions $\text{R}_2+\text{R}_3$ indicates model $B$'s output is within $\mathbb Z$. The number of inputs R3 is used to normalize statistics when enumeration is impossible (Sec.~\ref{sec:normalization}).  
% (d) We feed all the inputs sampled by $A$ (all \mytri) to both models to compute $\diff=z_{A,\mathbf{x}}-z_{B,\mathbf{x}}$. We collect the total count for each $\diff$ for the distribution $\rho_{A\rightarrow B}(\diff)$ (red histogram). The same procedure for model B generates $\rho_{B \rightarrow A}(\diff)$ (blue histogram). The ``x=x+1'' (\mycircle) is mapped to a very negative $\diff$ value because it has a small $z_{A,\mathbf{x}}$ but a large $z_{B,\mathbf{x}}$.
